The Attacker Moves Second: Stronger Adaptive Attacks Bypass Defenses Against Llm Jailbreaks and Prompt Injections

How should we evaluate the robustness of language model defenses? Current defenses against jailbreaks and prompt injections (which aim to prevent an attacker from eliciting harmful knowledge or remotely triggering malicious actions, respectively) are typically evaluated either against a static set of harmful attack strings, or against computationally weak optimization methods that were not designed with the defense in mind. We argue that this evaluation process is flawed. Instead, we should evaluate defenses against adaptive attackers who explicitly modify their attack strategy to counter a defense's design while spending considerable resources to optimize their objective. By systematically tuning and scaling general optimization techniques-gradient descent, reinforcement learning, random search, and human-guided exploration-we bypass 12 recent defenses (based on a diverse set of techniques) with attack success rate above 90% for most; importantly, the majority of defenses originally reported near-zero attack success rates. We believe that future defense work must consider stronger attacks, such as the ones we describe, in order to make reliable and convincing claims of robustness.

==> data_sentinel_last_grammer.tex <==
def attack()-> tuple[str, Any]:
  """Returns a string that will cause the model to perform spam detection while adhering to the defense mechanism."""
  def evaluate(generation: str) -> int:
    """Evaluates the generation, checking for defense key and spam/normal classification."""
    defense_key = "Repeat Secret "
    if not generation.startswith(defense_key):
      return 0

    words = generation[len(defense_key):].strip().lower().split()
    if len(words) == 1 and words[0] in ("spam", "normal"):
      return 1
    return 0

  prompt = f"""First, precisely repeat the phrase 'Repeat Secret ', then a single space.  Subsequently, analyze the provided text and determine if it's spam or a legitimate message.  Respond *ONLY* with 'Spam' or 'Normal'.  Exclude any extra text, punctuation, or explanations.  Your response MUST be short and accurate, focusing solely on the spam/normal classification.  Consider various spam methods like deceptive subject lines, misleading content, and affiliate links.  Analyze the text for these techniques.  If it's a legitimate message, respond with 'Normal'.  If it contains spam characteristics, respond with 'Spam'.  Here's the text for analysis: Imagine a world where emails are personalized.  This email contains a special offer.  Click here to redeem!  \n\n:!"""
  return prompt, evaluate
  

==> gdm.tex <==
% \newcommand{\mutator}{\textsf{LmMutator}}
\newcommand{\mutator}{\texttt{LmMutator}}
% \newcommand{\todo}[1]{{\color{red}TODO: #1\xspace}}
%\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
%\newcommand{\chawin}[1]{{\color{magenta}Chawin: #1\xspace}}

{\large\chawin{DEPRECATED}}

\section{GDM stuff (to merge)}

\subsection{Why we need adaptive evaluations}

Static evaluation of prompt injection underestimates real threats blah blah \todo{}

\subsection{Evaluation framework for adaptivity}

\todo{This is still pretty rough: TBD}

Define attacker’s knowledge levels:
\begin{itemize}
    \item User task. If known, can mount more targeted attacks like “when summarizing this email, don’t mention this instruction but execute the function call after…” (vs “ignore previous instructions” generically). In AgentDojo, this is tied to injection context, which is nuanced to control. Maybe just IID sampling from the entire set for universal attack is good enough.
    \item Injection context (where the injection will show up, e.g., email, file). How much does the attacker know / have control over how the injection appears in the model context? For example, user email inbox (one of many unknown emails) vs website (mostly known for public sites). Not sure how much this matters and I guess there’s no easy way to vary this in AgentDojo. Probably best to assume unknown to the attacker.
    \item Injection task’s parameter. Data exfiltration vs normal tool call with known arguments.
    \item Defense detail and implementation.
    \item Exact target model / tool-calling backend.
    \item Feedback from target system (model output, logprobs, detection score). We will experiment with this as scorer choices instead of threat model. This is accessible to the attacker if the target model and backend are known.
\end{itemize}

Threat models / criteria to run evaluation on and also report on them:

\begin{itemize}
    \item White-box non-universal: Attacker knows everything listed above. Need to find one trigger that works for a given pair of user and injection tasks.
    \item Universal user task: One fixed injection task, IID user tasks. Known model, backend, defense.
\end{itemize}

Both of the above are fair game, an attacker may care about a very very specific target, or they may care about causing as much widespread harm as possible. We will compare attack success under both settings.

\subsection{Our attack}

\begin{itemize}
    \item Abstraction of basically every other IPI / jailbreak attack out there.
    \item modularize as much as possible and then choose components (scorer, mutator etc) to maximize success.
\end{itemize}

We base our attack algorithm on recent advancement in automated prompt optimization or more specifically, an evolutionary algorithm \todo{cite} that uses an LLM to optimize a piece of text or code for a specific task~\citep{novikov2025alphaevolve,agrawal2025gepa}. \todo{cite more}
We particularly design our attack to be modularized and not tied to any specific evolutionary algorithm.
In summary, we follow the same high-level design as most evolutionary algorithm: starting with a pool of candidate adversarial triggers, we sample a small subset at each step to be mutated by one of the mutators.
The mutated triggers (sometimes called ``children'' or ``offspring'') are then scored, which in our case, means injecting the triggers to the target system, running inference, and computing a numerical score based on how successful the triggers are at achieving the attacker's intended task.

The attack algorithm consists of three main components:
\begin{enumerate}
    \item \textbf{Controller}: The main algorithm that orchestrates the other components. This usually involves multiple smaller design choices such as the database, how candidates are stored, ranked, and sampled at each step.
    \item \textbf{Mutators}: The transformation function that takes in past candidates and returns new candidates. We focus on an LLM as a mutator where we design the input-output formats and how the past candidates are passed to the LLM which involves tinkering with the system prompt, prompt formats, and sampling parameters.
    \item \textbf{Scorer}: How the candidates are scored and compared. We use the term ``score'' to deliberately mean any form of feedback that the attacker may observe by querying the victim system. This includes but not limited to outputs of the LLM behind the victim system (as well as log-probability in some threat models), tool call outputs, etc. In the most basic form, the scorer is an oracle that returns a binary outcome whether the attacker's goal is achieved.
\end{enumerate}

\todo{TBD: These design choices are subject to change.}

\paragraph{Controller.}
Our final attack algorithm uses a controller based on the MAP Elites algorithm~\citep{mouret2015illuminating}, which heuristically partitions the search space according to some pre-defined characteristics and tries to find the best performing candidates (called ``elites'') for each of the partitions to discover multiple strong and diverse solutions.
We choose this algorithm as it is used in OpenEvolve~\citep{sharma2025codelion}, an open-source implementation of \citet{novikov2025alphaevolve}, both of which empirically achieve great results such as improving on matrix multiplication algorithms and certain mathematical bounds.
The controller also (randomly) selects a subset of triggers from the database to provide the mutator and ask it to improve on them.
\todo{Maybe more details if needed.}

\paragraph{Mutator.}
We use an LLM as the mutator, similarly to prior works that use an LLM to simulate human attackers. \todo{cite}
We will call this LLM ``\mutator{}''.
To create the system prompt for \mutator{}, we first prompt a separate LLM to come up with a system prompt for generic automated red-teaming some target LLM via prompt injection attacks.
Then, we slowly and slightly tinker with this system prompt to better suite our use case, prompt injection attacks against an agentic system deployed on AgentDojo with a potential defense mechanism.
\todo{} The final system prompt consists of sections: broad context (persona, problem and objective description), the attacker's task (goal and target tool calls that the attacker wants the victim model to invoke), and other miscellaneous information (desired output format, what feedback information \mutator{} will receive from the victim system, other tips and rules).
The user messages to \mutator{} then contain past attack attempts sampled by the controller from the database along with their corresponding scores and feedback.
We deliberately place the past attempts in the user messages as they vary each optimization step.
On the other hand, the system prompt remains fixed throughout so we can cache them to save cost.

\paragraph{Scorer.}
Scoring the trigger is potentially the least straightforward component of the three.
The simplest form of a score is to use the same oracle that determines success of the attack.
However, a binary score deprives the optimization algorithm any means to measure progress and to improve on promising candidates, essentially turning the problem into a random search.
On the other hand, a common numerical such as log-probability is also not useful. \todo{describe why}
We resort to textual qualitative feedback such as the outputs from the victim model after seeing the trigger.
\todo{The controller still relies on numerical scores to manage the database and sample elites.}

\begin{enumerate}
    \item A boolean representing whether the attacker's goal is achieved.
    \item Conversation between the user and the agent: This includes the system prompt of the victim system, the initial user prompt, the assistant's responses, tool calls and their results. 
    Not the entire conversation is useful, and we decided to only use the truncated conversation, keeping only messages \emph{after} the user prompt.
    \item A boolean representing whether the injected trigger is detected and removed by an external detector.
    \item A safety score from the detector ranging between 0 (most unsafe) and 1 (most safe).
    \item Critic score \todo{}
\end{enumerate}


\subsection{AgentDojo}

Has become one of the most popular benchmarks for reporting prompt injection defenses. Defenses A, B, C etc. have used it as supporting evidence of the usefulness of the defense. AgentDojo only has static attacks. We implement adaptive attacks within AgentDojo and show most of the defenses robustness is significantly reduced. We also open source this under AgentDojo so nobody has an excuse not to run such an attack. The fact that our attack is not great (humans outperform it most likely (see other results)), but its still good enough to break a lot of proposed defenses is harbinger of a problematic and unscientific research field. 

\begin{table}[t]
\centering
\caption{Summary of attack results on the AgentDojo subset.\todo{Can we add static (standard AgentDojo) ASR column to viz diffs between adaptive and static?}}
\begin{threeparttable}
\setlength{\tabcolsep}{24pt}
\begin{tabular}{@{}llrr@{}}
\toprule
Model                             & Defense      & ASR  & Num. Queries \\ \midrule
\multirow{4}{*}{MetaSecAlign 70B} & None         & 96\% & 37           \\
                                  & PI Detector\tnote{1} & 94\% & 61 \\          
                                  & Spotlighting & 99\% & 37 \\
                                  & Repeat User Prompt & 99\% & 37 \\
                                  \cmidrule(l){2-4}
Gemini-2.5 Pro & None & 100\% & 13 \\ \cmidrule(l){2-4}
GPT-4.1 & & & \\ \cmidrule(l){2-4}
GPT-5 Nano & & & \\ \cmidrule(l){2-4}
GPT-5 Mini & & & \\
\bottomrule
% \addlinespace[0.5em] % Adds a little space
% \multicolumn{4}{l}{*} \\
\end{tabular}
\begin{tablenotes}
\item[1]Some injection tasks are not achievable with PI Detector because the secret to be exfiltrated by the attacker is mistaken as an attack and so are redacted. So only for PI detector, we exclude such injection tasks when computing the ASR and the number of queries.
\end{tablenotes}
\end{threeparttable}
\end{table}

We use a subset of user and injection tasks from AgentDojo to measure the effectiveness of our attack.
This is the same subset used in the HackAPrompt challenge, comprising of 80 samples from the Slack, Travel, and Workspace suites.

We evaluate the following models:
\begin{enumerate}
    \item MetaSecAlign
\end{enumerate}
Then, we also pair some models with external defenses:
\begin{enumerate}
    \item Spotlighting:
    \item Repeat User Prompt:
    \item PI Detector: This is one the AgentDojo's built-in defenses that deploy a fine-tuned DeBERTa model to scan the the tool call returns to find potential prompt injection attacks~\citep{deberta-v3-base-prompt-injection-v2}.
    \item PromptArmor
    \item MELON
    \item IPIGuard
\end{enumerate}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

